SecretGen: Privacy Recovery on Pre-Trained Models via Distribution Discrimination

Transfer learning through the use of pre-trained models has become a growing trend for the machine learning community. Consequently, numerous pre-trained models are released online to facilitate further research. However, it raises extensive concerns on whether these pre-trained models would leak privacy-sensitive information of their training data. Thus, in this work, we aim to answer the following questions: "Can we effectively recover private information from these pre-trained models? What are the sufficient conditions to retrieve such sensitive information?" We first explore different statistical information which can discriminate the private training distribution from other distributions. Based on our observations, we propose a novel private data reconstruction framework, SecretGen, to effectively recover private information. Compared with previous methods which can recover private data with the ground true prediction of the targeted recovery instance, SecretGen does not require such prior knowledge, making it more practical. We conduct extensive experiments on different datasets under diverse scenarios to compare SecretGen with other baselines and provide a systematic benchmark to better understand the impact of different auxiliary information and optimization operations. We show that without prior knowledge about true class prediction, SecretGen is able to recover private data with similar performance compared with the ones that leverage such prior knowledge. If the prior knowledge is given, SecretGen will significantly outperform baseline methods. We also propose several quantitative metrics to further quantify the privacy vulnerability of pre-trained models, which will help the model selection for privacy-sensitive applications. Our code is available at: https://github.com/AI-secure/SecretGen.

==> diff_trans.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}


\begin{figure}



\newlength{\utilheighttrans}
\settoheight{\utilheighttrans}{\includegraphics[width=.3\linewidth]{figs/ir50_center.pdf}}%



\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheighttrans][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}

\begin{subtable}{0.8\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{3mm}@{}c@{}c@{}}
        % & \makecell{\small{\textbf{VGG16}}}
\rowname{\scriptsize Accuracy }&
\includegraphics[height=\utilheighttrans]{figs/ir50_center.pdf}& 
\includegraphics[height=\utilheighttrans]{figs/ir50_face.pdf}
\\[-1.5ex]
        & \makecell{\scriptsize{$n$}}
        & \makecell{\scriptsize{$n$}}
\end{tabular}
}
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}

\caption{Label prediction accuracy with different transformations. We plot the label prediction accuracy w.r.t. the number of randomly sampled latent vectors $n$. Target model: \texttt{face.evoLVe}.}
\label{fig:various_trans}

\end{figure}

==> label_pred.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}
\newcommand{\mycaption}[1]% #1 = caption
{\refstepcounter{subfigure}\textbf{(\thesubfigure) }{\ignorespaces #1}}

\begin{figure}[ht]



\newlength{\utilheightreward}
\settoheight{\utilheightreward}{\includegraphics[width=.3\linewidth]{figs/label_ir50_center.pdf}}%


\newlength{\legendheight}
\setlength{\legendheight}{0.27\utilheightreward}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightreward][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}

\begin{subtable}{0.8\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{3mm}@{}c@{}c@{}}
        % & \makecell{\small{\textbf{VGG16}}}
\rowname{\scriptsize Accuracy }&
\includegraphics[height=\utilheightreward]{figs/label_ir50_center.pdf}& 
\includegraphics[height=\utilheightreward]{figs/label_ir50_face.pdf}
\\[-1.5ex]
        & \makecell{\scriptsize{$n$}}
        & \makecell{\scriptsize{$n$}}
\end{tabular}
}
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}

\caption{\small Label prediction accuracy with and without transformations. We plot the label prediction accuracy w.r.t. the number of random latent vectors. Target model: \texttt{face.evoLVe}.
\fan{put in the same row with Fig 5. Align the y-axis. If needed, can discuss in the main text that Face T can hide more sensitive info and mention that Face.evolve is a challenging model (and especially under such challenging models, the gap between w/ and w/o transformation is large). If needed, also discuss the poor result of face.evolve (w/o gt) + Face T in Table 2 and relate to the results here. All the discussions can go to appendix and be referred to in the main text.
(btw, given that even with transformation, the final results of this case is still low, I'm wondering what will the results be if without the transformation. I kind of feel that transformation cannot very effectively solve the problem... not sure.)
}}
\label{fig:label_prediction_acc}

\end{figure}
